ROOT for the HL-LHC: data format

This document discusses the state, roadmap, and risks of the foundational components of ROOT with respect to the experiments at the HL-LHC (Run 4 and beyond). As foundational components, the document considers in particular the ROOT input/output (I/O) subsystem. The current HEP I/O is based on the TFile container file format and the TTree binary event data format. The work going into the new RNTuple event data format aims at superseding TTree, to make RNTuple the production ROOT event data I/O that meets the requirements of Run 4 and beyond.

==> lhcc-root-foundation.pandoc.tex <==
\hypertarget{root-foundation-v1.1-2021-09-09}{%
\section{ROOT Foundation v1.1
{[}2021-09-09{]}}\label{root-foundation-v1.1-2021-09-09}}

This document discusses the state, roadmap, and risks of the
foundational components of ROOT with respect to the experiments at the
HL-LHC (Run 4 and beyond). As foundational components, the document
considers in particular the ROOT input/output (I/O) subsystem. The
current HEP I/O is based on the TFile container file format and the
TTree binary event data format. The work going into the new RNTuple
event data format aims at superseding TTree, to make RNTuple the
production ROOT event data I/O that meets the requirements of Run 4 and
beyond.

\hypertarget{characteristics-of-the-hep-io-format}{%
\subsection{Characteristics of the HEP I/O
format}\label{characteristics-of-the-hep-io-format}}

ROOT provides the common file format for the data of all the LHC
experiments, currently hosting more than 1EB of LHC data. WLCG estimates
a yearly cost of 50MCHF for storage alone. As such, a robust and
efficient ROOT I/O is central to the success of the HL-LHC physics
programme. Improvements such as improved compression, faster reads and
writes, and more reliable APIs benefit directly all the LHC experiments.

Given the projected volume of tens of exabytes and a life-time of HL-LHC
data of several decades, it is natural and cost-effective to use a
common I/O format that guarantees a lifetime compatible with HL-LHC. A
stable I/O format is also key to the long-term preservation of
experimental results. It is therefore crucial to retain expertise on I/O
software and technology in the HEP community.

The different stages of the data flow---data taking or simulation,
reconstruction, and analysis---come with different characteristics and
requirements to the I/O. Data taking puts a focus on fast writing and
the ability to recover gracefully from unexpected premature termination
of output streams. Reconstruction requires good interplay with
multi-threaded frameworks, support for a rich event data model (EDM),
and fast merging of multiple data streams from concurrent processing.
Analysis requires fast, selective reads both in terms of reading subsets
of the events (``skimming'') and in terms of reading subsets of the
collections and object properties in an event (``stripping'',
``slimming'' and ``thinning''). These requirements define a set of
essential properties for the I/O and distinguish HEP-I/O from general
purpose I/O as provided by other libraries and formats.

\hypertarget{essential-properties}{%
\subsubsection{Essential Properties}\label{essential-properties}}

The ROOT I/O library aims at providing the following essential
properties:

\begin{itemize}
\item
  \begin{quote}
  \textbf{Robustness}. Protection against reading of corrupted data.
  This includes both protection against corruption on the storage or
  transfer level, and accidental misuse of the data access API.
  \end{quote}
\item
  \begin{quote}
  \textbf{Stability}. In order to support long-term data preservation,
  the I/O library supports mechanisms for backward and forward
  compatibility. This enables the evolution of its binary format (within
  limits) as well as schema evolution of the serialized objects: ROOT
  I/O will translate for instance a jet read from an old file, to match
  the jet object in today's code. The I/O software development process
  prioritizes long-term maintenance and sustainable code design.
  \end{quote}
\item
  \begin{quote}
  \textbf{Expressiveness}. HEP data are naturally represented as a large
  number of stochastically independent, structured events. Events
  contain in turn collections of objects of (often significantly)
  varying sizes.
  \end{quote}
\item
  \begin{quote}
  \textbf{Usability}. The I/O library is used both by software experts
  and by novice programmers, making reading and writing of data
  accessible to novice programmers. In particular, arrays of C++ and
  Python objects in memory can be directly (de-)serialized to disk
  without an explicit schema definition by the user.
  \end{quote}
\item
  \begin{quote}
  \textbf{Speed}. The columnar layout of the ROOT event data format and
  the ROOT I/O scheduler are tuned for the HEP use cases, especially for
  sparse reading and merging of data. For these use cases, the ROOT I/O
  is faster than potential alternatives such as HDF5 or parquet {[}2{]}.
  \end{quote}
\item
  \begin{quote}
  \textbf{Concurrency}. Data is commonly accessed in the context of
  concurrent applications. The data format needs to be structured to
  facilitate inter- and intra-event parallelism. The I/O layer itself
  can also deploy concurrent algorithms such as compression.
  \end{quote}
\item
  \begin{quote}
  \textbf{Integration}. Data (de-)serialization is an integral part of
  the experiment computing workflows. The data format allows for storing
  experiment-specific and data management specific meta-data and
  integrates well with the experiment computing models.
  \end{quote}
\end{itemize}

The HL-LHC requirements on performance and efficient use of space in
combination with the essential non-functional properties cannot be found
in any single alternative format {[}2{]}.

\hypertarget{overview-of-the-io-components}{%
\subsection{Overview of the I/O
Components}\label{overview-of-the-io-components}}

Several noteworthy components and classes collectively make the ROOT I/O
library. Besides core components maintained by the ROOT team, the ROOT
I/O library delegates functionality such as remote data access and
authentication to the community's 3rd party implementations of choice.

\hypertarget{io-components-in-the-root-core-software}{%
\subsubsection{I/O Components in the ROOT Core
Software}\label{io-components-in-the-root-core-software}}

The ROOT core software contains classes to read and write event data, as
well as higher-level components for I/O scheduling, caching, and data
reflection.

The TTree classes currently define the low level data format and data
access API for LHC event data. TTree uses a columnar on-disk layout. It
is used for all data product stages, from raw data to final-stage
ntuples, and is the core property and benefit of ROOT's current I/O
format, a data layout that is now adopted by many other "big data"
tools.

The TFile container format allows to store TTree data, RNTuple data and
non-event data such as histograms in a single file. The TFile format
provides backward and forward compatibility over decades.

The RNTuple classes are the designated successor of the TTree classes.
Based on more than 25 years of experience with TTree and inspired by
advances in I/O algorithms and hardware in industry and academia,
RNTuple introduces a new data format and new data access APIs. The
format and the APIs are backwards incompatible to TTree. This one-time
compatibility break allows for the necessary flexibility in harnessing
space savings, increasing the read/write speed, and improving the
robustness of the API for the decades to come. RNTuple includes an I/O
scheduler that optimizes and parallelises the read requests for local
devices (HDD, SSD) and remote storage (XRootD, HTTP, object stores,
network file systems). RNTuple includes the RNTupleLite library that
provides low-level access to uncompressed data buffers through a C API
and is independent of ROOT's core library. The RNTuple binary format is
specified to facilitate future 3rd party implementations, should the
need arise.

ROOT's C++ and Python reflection capabilities are central to the I/O
system; they enable serialization of user-defined objects. This type
description is using ROOT's interpreter cling, which in turn utilizes
the state-of-the-art C++ compiler libraries clang/llvm. Following
clang's development for instance in support of new C++ standards allows
cling and thus ROOT I/O to "understand" modern C++ code, not limiting
the experiments in their expressiveness. The serialization of events
into the columnar on-disk layout effectively implements an AoS (array of
struct) to SoA (struct of array) transformation at the I/O layer that is
shared by all the RNTuple users.

Several higher-level I/O components provide support for specific use
cases. In particular, ROOT provides support for application-defined data
caching (TFilePrefetch) and dedicated support for multi-threaded and
multi-node merging of partial results (TBufferMerger).

\hypertarget{plugins-and-3rd-party-components}{%
\subsubsection{Plugins and 3rd Party
Components}\label{plugins-and-3rd-party-components}}

The ROOT core I/O integrates with the following 3rd party components
that are important for the I/O of HL-LHC experiments

\begin{itemize}
\item
  \begin{quote}
  Remote access protocols: XRootD is critical for the production
  workflows; Davix is used for HTTP access and in particular for
  training, outreach and open science
  \end{quote}
\item
  \begin{quote}
  Authentication plugins, namely X.509 certificates and SciTokens
  \end{quote}
\item
  \begin{quote}
  Compression algorithms and lossy compression schemes; RNTuple and
  TTree provide the means to use both classes of compression
  \end{quote}
\item
  \begin{quote}
  Connectors to efficiently accommodate new "beyond file system" storage
  (for instance Intel DAOS object store and Amazon S3 compliant cloud
  storage) and "beyond grid" compute resources such as exascale HPCs and
  clouds.
  \end{quote}
\end{itemize}

\hypertarget{requirements-from-hl-lhc-experiments}{%
\subsection{Requirements from HL-LHC
Experiments}\label{requirements-from-hl-lhc-experiments}}

Compared to Run 1-3, we expect a tenfold increase in the number of
events for HL-LHC. While the exact effect of the increased data influx
on file sizes and number of files is currently under investigation (see
DOMA document), the file format needs to be prepared to handle
significantly larger files and for a more flexible combination of
physical files to virtual data sets. That puts stronger robustness
requirements on the I/O layer, e.g. for keeping data provenance
information, for checksumming data and for the error handling of device
failures. In line with the experiment efforts on creating very compact
analysis object formats, ROOT optimises the I/O performance especially
for simple EDMs with structures of fundamental data types ("plain-old
data") and collections thereof {[}6, 10{]}.

On the level of the computing model, remote I/O has already become a
standard data access mode, a trend that will intensify towards HL-LHC
(see also DOMA efforts). HPC systems and clouds play an increasing role
as resources beyond the standard grid. These resources come with their
own (remote and/or distributed) storage access technologies: cluster
file systems and high-performance object stores for HPC sites, S3-like
HTTP based object stores with URL based signatures and tokens for
clouds. These storage types are expected to be increasingly used as
temporary or tactical storage for LHC data. In addition, some data is
expected to be stored on a new, ``volatile'' storage class built from
out-of-warranty drives for best use of existing resources, emphasising
the need for rigid checksums on the file format level.

The increasing use of machine learning training and inference has an
impact on storage, too. The I/O system has to provide fast data pipes of
event data to GPUs and other accelerators, ideally without involving the
host CPU for the transfer. Here, ROOT's columnar data is a perfect data
layout for GPU acceleration.

\hypertarget{evolution-of-the-technology-landscape}{%
\subsection{Evolution of the Technology
Landscape}\label{evolution-of-the-technology-landscape}}

The TTree I/O container was designed based on the hardware of the 1990s.
Meanwhile, the technology landscape has changed significantly, with
generally greater architectural heterogeneity. The boundaries between
network, permanent storage, memory, and compute devices are blurring
{[}1{]}. Remote storage is the norm rather than an exception, with
varying degrees of remoteness and abstractions. And compute devices are
ever more parallel and specialised.

\hypertarget{ultra-fast-storage-devices}{%
\subsubsection{Ultra-Fast Storage
Devices}\label{ultra-fast-storage-devices}}

Modern I/O devices such as 100GbE network cards and 10GB/s NVMe disks
closely match the throughput of a CPU core. As a result, I/O code paths
must be highly CPU optimized. In contrast to spinning disks with few
platters, SSDs provide their full performance only when concurrently
accessing tens or hundreds of cells. Furthermore, a new class of
flash-based storage devices supports byte-addressed access as opposed to
block-level access, which requires explicit support from the I/O layer
to harness their full potential. Byte-addressable storage devices are
already deployed for some performance-critical applications (e.g.
databases, HPC object stores) and may become part of the standard HEP
storage hierarchy on the HL-LHC timescale.

\hypertarget{parallelism-and-accelerators}{%
\subsubsection{Parallelism and
Accelerators}\label{parallelism-and-accelerators}}

TTree originally assumed single-core nodes, whereas HL-LHC's typical
core counts will surpass 100 cores per box. The I/O is now embedded in
multi-threaded frameworks and makes active use of multithreading itself,
for instance for data compression and decompression. Standard
environments increasingly deploy GPUs, used to offload for instance
machine learning, tracking, and fitting tasks. GPUs have a memory model
different from CPUs and support new, reduced precision floating point
layouts, which benefit from dedicated support by the I/O layer.

Some storage systems provide specific computational capabilities
(``active storage''), e.g. for compression and checksumming {[}5{]}.
Active storage requires tight integration with the I/O application layer
to use its capabilities.

\hypertarget{distributed-and-remote-storage}{%
\subsubsection{Distributed and Remote
Storage}\label{distributed-and-remote-storage}}

Besides local and remote POSIX file system access, the I/O for HL-LHC
needs to be prepared for file-less storage systems such as distributed
object stores. The scalability limits of the POSIX API make file-less
storage systems ever more popular. Cloud storage is already dominated by
S3-like object stores, and HPC sites will likely rely on object stores
for the next-generation supercomputers {[}8{]}. With the divergence from
the standard POSIX API and paradigms, however, a variety of data access
APIs have emerged with no clear winner yet. As a result, I/O software
for HL-LHC needs to retain the flexibility to adapt, and a design that
allows this adaptation with minimal cost, with respect to both
performance and sustainability.

Even within the POSIX universe, applications can exploit an increasing
number of tunable parameters by harnessing the actual file system's
idiosyncrasies. Ceph-FS for instance, which is used as a shared HPC
cluster file system at CERN and elsewhere, can achieve improved
performance by tuning custom file metadata.

\hypertarget{ttree-plans}{%
\subsection{TTree Plans}\label{ttree-plans}}

With the heritage of more than 1EB of LHC data, the TTree file format
will remain supported in ROOT in parallel to the new RNTuple
developments. TTree also provides the baseline for RNTuple with respect
to performance and functionality. However, the priority in the TTree
support will shift to long-term data preservation. At the time scale of
HL-LHC, TTree won't benefit from the increased and shared expertise and
effort that RNTuple receives.

Tool support for disk-to-disk conversion from TTree to RNTuple is
underway and expected for 2021. Large-scale conversion of data, e.g.
using spare I/O cycles, is conceivable according to experiments' needs
as of the production release expected for 2024. Alternatively, archived
TTree datasets may be converted on the fly when reading from tape.

\hypertarget{rntuple-potential-and-roadmap}{%
\subsection{RNTuple Potential and
Roadmap}\label{rntuple-potential-and-roadmap}}

The RNTuple I/O system is a multi-year effort to evolve to ROOT event
data I/O for the challenges of the upcoming decades. It comes with a
rich R\&D programme on a compact data format, on performance engineering
for modern storage hardware, on robust interfaces that are easy to use
and hard to use incorrectly, and on various other I/O aspects {[}3,
4{]}. RNTuple is also an opportunity to grow the next generation of the
community's long-term I/O experts.

RNTuple provides best performance for typical HEP use cases. It aims to
closely match the I/O device speed, sustaining at least 10GB/s per box
and 500MB/s per core for typical analysis throughput on the current
generation of hardware and scaling up with the increased performance of
new hardware. To this end, RNTuple avoids virtual function calls and
branches in hot code paths. It is also designed for providing direct
access to the I/O data buffers for zero-copy and bulk I/O. On fast
storage devices, RNTuple already shows 2-5 times better single-core
performance than TTree {[}3{]}. RNTuple is also designed for better
scaling to high core counts. The memory management is based on pages
rather than on TTree ``baskets''. Pages have a fixed size of O(100kB)
independent of the event sizes, which allows for more fine-grained
parallelism and prevents a negative memory impact of large outlier
events.

The RNTuple classes are conditionally thread safe (i.e., they use no
globals or statics) and thus work well in multi-threaded applications.
Asynchronous, parallel I/O is the default. RNTuple uses parallel range
requests for remote storage (XRootD, HTTP) and local storage. This
approach optimally uses parallel storage devices such as SSDs and
overlaps computation and data access. Optionally, RNTuple connects to a
task scheduler (e.g. Intel TBB) for transparent, task-parallel
compression and decompression of pages. The code is designed to allow
for later offloading of compression to dedicated devices.

Compared to TTree, RNTuple has a significantly more compact data
representation. Comparisons show 15\% (lzma) - 25\% (zstd) smaller files
after compression with files from ATLAS, CMS, and ALICE. The space
savings are due to a very compact representation of (nested) collections
and various smaller optimizations. The introduction of the new RNTuple
format also allows for changing the default compression algorithm from
zlib to the better zstd. Ongoing R\&D investigates lossy compression
schemes; any benefits will come on top of the other savings. Given the
50MCHF/year currently invested in WLCG storage, the community can
benefit from considerable cost savings and higher luminosity exposed to
analyses.

RNTuple has a 4-layered architecture: data access API, serialisation of
C++ objects, management of storage-backed vectors of simple types, and
the storage of byte ranges. The layer separation facilitates adaptation
to file-less storage systems {[}9{]}. The byte range layer is prepared
to work with byte-addressable as well as traditional block-based storage
devices. The explicit translation of C++ objects into arrays of simple
types allows for robust data interpretability even in the absence of C++
reflection capabilities. For instance, 3rd party tools can interpret the
structure and (within limits) the meaning of RNTuple data without an
understanding of C++ classes, as has been recently demonstrated in the
context of research on a memory layout abstraction library {[}7{]}.

The RNTuple API follows modern C++ core guidelines to provide a robust
interface to users. It uses smart pointers for a clear pointer
ownership. There are compile-time type-safe APIs for end-users and
type-unsafe APIs with runtime checks for frameworks. The systematic use
of exceptions prevents silent I/O failures and silently corrupted data.
On the file format level, data and meta-data are systematically
checksummed to guarantee data integrity against corruption due to
storage devices or network transfers.

Like TTree, the programming model is designed for the needs of the HEP
community, which is hard to achieve with industry standard tools. In
particular:

\begin{itemize}
\item
  \begin{quote}
  RNTuple is integrated as a data source with RDataFrame (see analysis
  chapter).
  \end{quote}
\item
  \begin{quote}
  RNTuple provides a flexible meta-data API that allows experiments to
  store physics meta-data such as scale factors, as well as allowing
  data management tools like Rucio to access and write certain
  meta-data.
  \end{quote}
\item
  \begin{quote}
  Like in TTree, vertical and horizontal data combinations are provided
  through friends and chains
  \end{quote}
\item
  \begin{quote}
  Like TTree, RNTuple provides seamless support for serializing C++ and
  Python objects through ROOT's reflection facilities, as provided by
  ROOT's C++ interpreter cling
  \end{quote}
\end{itemize}

Having full control of the I/O layer allows for further integration in
the future where needed. Integration targets may include data access and
authentication protocols, data management systems, Grid file transfer
services, or tuning for specific file systems and network interconnects
in HPC facilities.

\hypertarget{rntuple-development-timeline}{%
\subsubsection{RNTuple Development
Timeline}\label{rntuple-development-timeline}}

The RNTuple development is a major undertaking of the ROOT team. We
continue to solicit community support and contributions. We foresee
several milestones along the way to validate the approaches and
coordinate integration with experiment frameworks. The following
timeline is conceived for a stable RNTuple developer work force of 2.5
experienced full-time engineers (see analysis chapter).

\begin{itemize}
\item
  \begin{quote}
  2018-2019: Creation of the software architecture, R\&D on the binary
  file format, development of first prototypes
  \end{quote}
\item
  \begin{quote}
  2019-2020: Integration in ROOT::Experimental, performance validations
  \end{quote}
\item
  \begin{quote}
  2021:
  \end{quote}

  \begin{itemize}
  \item
    \begin{quote}
    First integration in experiment frameworks (nanoAOD output module
    for CMSSW)
    \end{quote}
  \item
    \begin{quote}
    Development of object storage backends (Intel DAOS, S3)
    \end{quote}
  \item
    \begin{quote}
    Development of the schema evolution mechanisms
    \end{quote}
  \item
    \begin{quote}
    Based on the experience of the prototypes, specification of the
    version 1 binary format
    \end{quote}
  \end{itemize}
\item
  \begin{quote}
  2022
  \end{quote}

  \begin{itemize}
  \item
    \begin{quote}
    Optimization of RNTuple integration with ROOT's analysis interface
    RDataFrame ("bulk processing")
    \end{quote}
  \item
    \begin{quote}
    Development of conversion tools, debug / inspection tools,
    facilitating the use and adoption of RNTuple
    \end{quote}
  \item
    \begin{quote}
    Training of experiments' core developers
    \end{quote}
  \item
    \begin{quote}
    Validation and of I/O type system completeness, in particular
    potentially missing STL types, opaque data types, references
    \end{quote}
  \end{itemize}
\item
  \begin{quote}
  2023
  \end{quote}

  \begin{itemize}
  \item
    \begin{quote}
    Large-scale benchmarking and optimization of experiments' uses of
    RNTuple
    \end{quote}
  \item
    \begin{quote}
    Development of automatic optimization features, such as
    branch-specific compression, prefetching and cache-reuse, page size,
    adjustment to storage-specific parameters (e.g. block size, queue
    depth)
    \end{quote}
  \item
    \begin{quote}
    Validation of reading and writing data on PB scale
    \end{quote}
  \end{itemize}
\item
  \begin{quote}
  2024: Training of physicists
  \end{quote}
\end{itemize}

\hypertarget{adoption-work}{%
\subsection{Adoption Work}\label{adoption-work}}

Besides the RNTuple development work itself, a successful community
adoption requires additional development and training efforts. This work
cannot be done by the ROOT team alone. In particular, it requires
investment from the experiments for the integration of RNTuple into
their software frameworks. To this end, integration efforts can be based
on the experience with a first CMSSW integration for the generation of
nanoAOD RNTuple files.

Furthermore, community support is required for training and
dissemination, as well as the validation and optimization of the RNTuple
I/O to cover the wide spectrum of usage contexts of ROOT I/O.

\hypertarget{risks}{%
\subsection{Risks}\label{risks}}

For the efforts to prepare the ROOT foundations for HL-LHC, we see the
following challenges:

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\item
  \begin{quote}
  Keeping the schedule of the RNTuple implementation plan which depends
  on the availability of the required development resources.\\
  The potential impact is a fragmentation of the community using
  several, ad-hoc I/O approaches (e.g. TTree, protobuf, etc.) and along
  with it the risk of increased storage needs and reduced compute
  efficiency. As a risk mitigation, we foresee the gradual rollout of
  RNTuple, starting from derived data products up to raw data. This
  allows directing development efforts to critical areas in an agile
  way, based on feedback.
  \end{quote}
\item
  \begin{quote}
  Long-term retention of TTree and RNTuple I/O experts.\\
  The potential impact is a trust erosion in the data format and
  inefficiencies due to workarounds. As a mitigation we consider a
  thorough code development and documentation process according to best
  practices as well as education and sharing of expertise through R\&D
  and adoption. We also consider the existing permanent positions
  invested in I/O an important risk mitigation.
  \end{quote}
\item
  \begin{quote}
  Optimal design of the RNTuple format and API for the hardware and
  software requirements for Run 4.\\
  The potential impact is a loss of performance, thus a limitation on
  the efficiency of HL-LHC computing workflows, and in the worst case
  partial data loss. Other risk dimensions include the lack of
  flexibility needed to address future challenges or evolving
  requirements, or unacceptable limitations of supported experiments'
  data formats. As a mitigation, we plan for involvement of the
  stakeholders in the RNTuple specification, validation tests with
  experiments, and best practices used during the development. The
  RNTuple design is informed by the TTree experience, allowing for
  adaptation in areas expected to change on the time scale of HL-LHC,
  such as object store technology and active storage.
  \end{quote}
\item
  \begin{quote}
  Availability of remote access protocol libraries.\\
  The availability of a well-maintained XRootD client library and its
  integration in ROOT is critical for the HEP community. The
  availability of a well-maintained Davix client library and its
  integration in ROOT is important for training, outreach, and open
  science. While not directly related to ROOT, HTTP library support is
  also critical for the HEP community for 3rd-party copies
  (storage-to-storage transfers).
  \end{quote}
\item
  \begin{quote}
  Optimization of experiments' persistent data model for RNTuple.\\
  The RNTuple design anticipates the ongoing optimization of the
  experiments' persistent data model. Investing in developer FTEs on
  both ROOT's and the experiments' side to ensure a close feedback loop
  between the ROOT team and experiments and for the early adoption by
  experiments is critical. We believe that benefits provided by RNTuple
  are sufficiently convincing to warrant the experiments' transition
  with high priority.
  \end{quote}
\item
  \begin{quote}
  Evolving ROOT reflection support.\\
  To accommodate the experiments' continuous demand for the always
  newest C++ standard, with its additional features, efficiency, and
  expressiveness, ROOT needs to have the ability to understand newest
  C++ code, to extract type description (reflection), and to serialize
  objects of these types. This requires excellent C++ support as
  provided by one of the few industry-grade C++ compilers and libraries,
  clang. Cling and ROOT must follow and ideally influence clang's steady
  yet fast-paced evolution, which requires very specialized expertise
  and dedicated, continuous effort. Expert effort is also required for
  evolving and supporting ROOT's type description system, and for
  providing stable interfaces in ROOT despite an ever changing clang,
  for the lifetime of HL-LHC's usage of C++.
  \end{quote}
\end{enumerate}

\hypertarget{bibliography}{%
\subsection{Bibliography}\label{bibliography}}

\begin{quote}
{[}1{]} Appuswamy, Raja, et al. ``The Five-Minute Rule 30 Years Later
and Its Impact on the Storage Hierarchy.'' \emph{Communications of the
ACM}, vol. 62, no. 11, 2019, pp. 114-120.

{[}2{]} Blomer, Jakob. ``A quantitative review of data formats for HEP
analyses.'' \emph{Journal of Physics: Conference Series}, vol. 1085, no.
3, 2018.

{[}3{]} Blomer, Jakob, et al. ``Evolution of the ROOT Tree I/O.''
\emph{EPJ Web Conf}, vol. 245, 2020, p. 02030.

{[}4{]} CERN. \emph{Strategic R\&D Programme on Technologies for Future
Experiments}. 2018, CERN-OPEN-2018-006.

{[}5{]} Do, Jaeyoung, et al. ``Programmable software-defined solid-state
drives can move computing functions closer to storage.''
\emph{Communications of the ACM}, vol. 62, no. 6, 2019, pp. 54-62.

{[}6{]} Elmsheuser, Johannes, et al. ``Evolution of the ATLAS analysis
model for Run-3 and prospects for HL-LHC.'' \emph{EPJ Web Conf}, vol.
245, no. 06014, 2020.

{[}7{]} Gruber, Bernhard Manfred, et al. ``LLAMA: The Low Level
Abstraction For Memory Access.'' \emph{CoRR}, vol. abs/2106.04284, 2021,
https://arxiv.org/abs/2106.04284.

{[}8{]} Lockwood, Glenn K., et al. ``Storage 2020: A Vision for the
Future of HPC Storage.'' \emph{Lawrence Berkeley National Laboratory},
no. LBNL-2001072, 2017.

{[}9{]} Lopez Gomez, Javier, and Jakob Blomer. ``Exploring Object Stores
for High-Energy Physics Data Storage.'' \emph{Proc. CHEP 21 (accepted)},
2021.

{[}10{]} Rizzi, Andrea, et al. ``A further reduction in CMS event data
for analysis: the NANOAOD format.'' \emph{EPJ Web Conf}, vol. 214, no.
06021, 2019.
\end{quote}

